Lagrangian Covector Fluid with Free Surface

This paper introduces a novel Lagrangian fluid solver based on covector flow maps. We aim to address the challenges of establishing a robust flow-map solver for incompressible fluids under complex boundary conditions. Our key idea is to use particle trajectories to establish precise flow maps and tailor path integrals of physical quantities along these trajectories to reformulate the Poisson problem during the projection step. We devise a decoupling mechanism based on path-integral identities from flow-map theory. This mechanism integrates long-range flow maps for the main fluid body into a short-range projection framework, ensuring a robust treatment of free boundaries. We show that our method can effectively transform a long-range projection problem with integral boundaries into a Poisson problem with standard boundary conditions -- specifically, zero Dirichlet on the free surface and zero Neumann on solid boundaries. This transformation significantly enhances robustness and accuracy, extending the applicability of flow-map methods to complex free-surface problems.

==> leapfrog_figure.tex <==
\newcommand{\leapfroghelper}[2]{
\hspace{-0.15cm}
    \begin{subfigure}[t]{#2\textwidth}
    \includegraphics[width=\linewidth]{imgs/leapfrog/previous/white/frame_000#1.jpg}
    \\
    \includegraphics[width=\linewidth]{imgs/leapfrog/our/white/frame_000#1.jpg}
   
    \end{subfigure} \hspace{-0.15cm}
}

\begin{figure*}[ht]
\hfill
\begin{minipage}[t]{0.45\textwidth}    
    \leapfroghelper{001}{.20}
    %\leapfroghelper{020}
    \leapfroghelper{041}{.20}
    %\leapfroghelper{062}
    \leapfroghelper{083}{.20}
    %\leapfroghelper{101}
    %\leapfroghelper{123}
    %\leapfroghelper{147}
    %\leapfroghelper{165}
    %\leapfroghelper{191}
    \leapfroghelper{210}{.20}
    %\leapfroghelper{227}
    %\leapfroghelper{260}

    \vspace{-0.25cm}
    \caption{Leapfrog vortices in 2D. PPM (\textit{top}), our approach (\textit{bottom}).}
    \label{fig:leapfrog_2d}
\end{minipage}
\hfill
\begin{minipage}{0.53\textwidth}
 \vspace{-0.25cm}
 \centering
  \includegraphics[width=0.43\columnwidth]{imgs/ablation_study_convergence/ablation_convergence_plot.png}
 \vspace{-0.35cm}
 \caption{ 
 %We show by subtracting the pressure gradient, the convergence rate and divergence error of our method our method get significantly reduced.
 The performance when using different flow map lengths is shown in the case of both the original Covector Fluid technique, and our method, where previous pressure integration is subtracted before projection. \textit{Blue, green}, and \textit{red} lines depict divergence error-interative step curve for conjugate gradient solver for poisson equation of flow map length 1, 8, and 17, respectively. \iffalse We observe an improved rate of convergence and reduced divergence error by subtracting the pressure gradient.\fi We observe an improved rate of convergence by our method.  This plot corresponds to Leapfrog example and convergence error is calculated by averaging $|\nabla\cdot \mathbf{u}|$ on particles.
 }\iffalse Revision 9\fi\iffalse Revision 10\fi
 \label{fig:ablation_convergence}
\end{minipage}

\end{figure*}

==> taylor_green_2d_figure.tex <==

\begin{figure}[htb]
  \centering 
  
  \begin{subfigure}[t]{.32\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{imgs/taylor_green_2d/previous/frame_000701.jpg}
    \caption{PPM}
    \label{fig:sub1}
  \end{subfigure}%
  \hfill
  \begin{subfigure}[t]{.32\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{imgs/taylor_green_2d/our/frame_000701.jpg}
    \caption{Our method}
    \label{fig:sub2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{.33\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{imgs/taylor_green_2d/taylor_green_plot_no_text.png}
    \caption{Volume-averaged kinematic energy (x-axis) over time steps (y-axis).}
  \end{subfigure}
  
  \caption{Qualitative and quantitative evaluation of simulating Taylor-Green vortices. (a) and (b) show the state for each method after $700$ time steps. (c) shows the energy dissipation for PPM (orange) and our method (blue) over $500$ time steps.
  \label{fig:taylor_green_2d}}
\end{figure}
